Synchronization and oscillation quenching in interacting metronomes on a movable platform: simple model and bifurcation analysis

Various oscillatory phenomena occur in the world. Because some oscillations are related to abnormal states (e.g., particular diseases), establishing state-transition methods from an oscillatory to a resting state is important. In this study, we construct a simple metronome model and analyze the oscillation-quenching phenomenon of metronomes on a platform as an example of such state transitions. Although numerous studies were conducted on the metronome dynamics, most of them focused on the synchronization, and few studies treated the oscillation quenching because of the difficulty in analysis. To facilitate the analysis, we model a metronome as a linear spring pendulum with an impulsive force (escapement mechanism) described by a fifth-order polynomial. By performing an averaging approximation, we obtain a phase diagram for the in-phase synchronization, anti-phase synchronization, and oscillation quenching. We also numerically integrate the equation of motion and confirm the agreement between the analytical and numerical results. Despite the simplicity, our model successfully reproduces essential phenomena in interacting mechanical clocks, such as the bistability of in-phase and anti-phase synchrony and oscillation quenching occurring for a large mass ratio between the oscillator and the platform. We believe that our simple model will contribute to future analyses of other dynamics observed in metronomes.

==> sub.tex <==


